Posterior Distillation Sampling

We introduce Posterior Distillation Sampling (PDS), a novel optimization method for parametric image editing based on diffusion models. Existing optimization-based methods, which leverage the powerful 2D prior of diffusion models to handle various parametric images, have mainly focused on generation. Unlike generation, editing requires a balance between conforming to the target attribute and preserving the identity of the source content. Recent 2D image editing methods have achieved this balance by leveraging the stochastic latent encoded in the generative process of diffusion models. To extend the editing capabilities of diffusion models shown in pixel space to parameter space, we reformulate the 2D image editing method into an optimization form named PDS. PDS matches the stochastic latents of the source and the target, enabling the sampling of targets in diverse parameter spaces that align with a desired attribute while maintaining the source's identity. We demonstrate that this optimization resembles running a generative process with the target attribute, but aligning this process with the trajectory of the source's generative process. Extensive editing results in Neural Radiance Fields and Scalable Vector Graphics representations demonstrate that PDS is capable of sampling targets to fulfill the aforementioned balance across various parameter spaces.

==> Sections/1_Introduction_v1.tex <==
\section{Introduction}
\label{sec:introduction}


For users to have full freedom in handling visual content, editing existing content is as important as creating new ones. Recently, the 2D image domain has witnessed swift progress in both text-driven generation~\cite{Saharia:2022IMAGEN,Rombach:2022StableDiffusion, Ramesh:2022DALLE2} and editing~\cite{Wallace:2023EDICT, Huberman:2023FriendlyInversion, Hertz:2023Prompt-to-Prompt, Wu:2023CycleDiffusion} using large-scale diffusion models~\cite{Rombach:2022StableDiffusion, Saharia:2022IMAGEN, Brooks:2023InstructPix2Pix, DeepFloyd, Midjourney, Ramesh:2022DALLE2}. Riding on this wave of huge success, many have explored using this rich prior of the 2D diffusion models for other parametric images~\cite{Poole:2023DreamFusion, Wang:2023SJC, Metzer:2023LatentNeRF, Jain:2023VectorFusion}. 

Poole~\etal~\cite{Poole:2023DreamFusion} first open the door to the generation of parametric images, specifically Neural Radiance Fields (NeRFs)~\cite{Mildenhall:2020NeRF}, using the 2D diffusion prior through an optimization named Score Distillation Sampling (SDS). Following Poole~\etal~\cite{Poole:2023DreamFusion}, various works have applied SDS not only in NeRF representations~\cite{Lin:2023Magic3D, Wang:2023ProlificDreamer, Shi:2023MVDream, Zhu:2023HiFA, raj2023dreambooth3d} but also in more diverse parametric spaces such as texture~\cite{Metzer:2023LatentNeRF, Anonymous:2023SDSTexturing}, material~\cite{Xu:2023MATLABER}, scalable vector graphics~\cite{Jain:2023VectorFusion}, sketches~\cite{Xing:2023DiffSketcher} and semantic typographics~\cite{Iluz:r2023Word-As-Image}. While SDS has proven successful in text-to-generation across different parametric spaces, it has not fully utilized the zero-shot capabilities of diffusion models for \emph{editing} in the parametric space, especially when compared to the advancements seen in the 2D image domain.

Unlike generation, the key aspects of text-driven editing are two-fold: (1) aligning with a target text and (2) preserving the unique identity of source content. While SDS successfully address the former, it lacks the latter aspect. To alleviate this issue, Hertz~\etal~\cite{Hertz:2023DDS} propose Delta Denoising Score (DDS) for editing tasks. DDS reduces the noisy gradients found in SDS, leading to background preservation and sharper outputs. However, DDS still does not have any explicit term for the identity preservation. To bridge this gap, we turn our attention to a recent 2D image editing algorithm, known as diffusion inversion. In this paper, we leverage the latent space from diffusion inversion, which encodes richer identity information, to adapt the SDS optimization for editing beyond simple noise matching.

As methods based on SDS have developed to utilize diffusion models in various parametric image generation tasks, diffusion inversion has also bloomed for 2D image editing. Its primary objective is to find the corresponding latent of an input image in diffusion models so that it can effectively regenerate the image through a generative process. Once the latent is computed, the original image can be edited by running the generative process with the computed latent and new conditions such as new target text prompts.

\Topic{DDPM Inversion}
Among various methods for diffusion inversion~\cite{Hertz:2023Prompt-to-Prompt, Dhariwal:2021ADM, Mokady:2023NullTextInversion, Wallace:2023EDICT}, recent works~\cite{Wu:2023CycleDiffusion, Huberman:2023FriendlyInversion} focus on the information encoded in the stochastic noise latent space of diffusion models. This noise latent space is from the posterior of a forward process of diffusion models. Unlike a noise prediction itself, the noise latent space encode both the source content information and the guidance direction of diffusion models. \Juil{Need to fill in the details.}

\Topic{Comparison to other NeRF editing papers}
Recent work has leveraged the 2D diffusion prior for NeRF editing. Their methods are generally divided into two approaches: (1) directly applying SDS optimization into NeRF parameters or (2) 
iteratively updating ground-truth images in the 2D space, called Iterative Dataset Update (Iterative DU), and adjusting NeRF to align with these updated images. For the first approach, a specific local editing region is required to be predetermined since the SDS optimization is prone to affect unintended regions, causing the results that significantly deviate from the original NeRF scene. Thus, they are restricted to localized edits and has difficulty handling extensive geometric deformations or adding objects in unspecific regions. On the other hand, the alternative approach~\cite{Haque:2023InstructNeRF, Mirzae:i2023WatchYourStep, Wang:2023InpaintNeRF360} based on Iterative DU processes editing in 2D image domain. They edit 2D rendering outputs and subsequently adapts NeRF parameters to match the updated images. However, for NeRF to converge in 3D space, edited images must meet consistency across different views. Consequently, these methods mainly focus on appearance changes, encountering challenges when edits could produce substantial inconsistent outputs across different views, such as large geometric changes or adding objects in unspecific regions.

\Topic{Strengths of our method}
To address the aforementioned challenges, we introduce a novel optimization method tailored for 
parametric image editing. We provide extensive experimental results to demonstrate the versatility of our method. When editing NeRF, our method directly updates NeRF parameters in the 3D space, thus bypassing the view inconsistency issues inherent to the iterative DU method. It enables not just appearance changes but also geometric deformations and the addition of objects in outdoor scenes which have not been tackled by previous work to our best knowledge. 
We also expand our editing experiments to the SVG domain. \Juil{Add SVG editing results later.} 
Furthermore, our optimization is pioneering in considering identity preservation term in SDS. We further provide a detailed analysis, comparing our optimization with DDS, and demonstrate it can be seen as a generalized form of DDS.

==> Sections/4_Method_v1.tex <==
\section{NeRF Editing with \Ours{}}
We introduce our overall pipeline for NeRF editing using \Ours{}. Given a set of paired real images and their corresponding camera parameters $\{(I_v, c_v)\}$ for viewpoint $v$, we first initialize a NeRF scene using the real images. To apply \Ours{}, a text prompt $y^{\text{src}}$ is also required that describes the real images. However, we observed there are some inconsistencies between an ideal text prompt, which would ideally reproduce the input image through the generative process, and the actual prompt we provide. To alleviate this discrepancy issue, we have found that it is effective to finetune a pre-trained model with $\{I_v\}$ and $y^{\text{src}}$ following the DreamBooth~\cite{Ruiz:2023DreamBooth} setup.

\label{sec:method}
\paragraph{\Ours{} Optimization Stage.}
After the NeRF initialization, we update the NeRF scene using \Ours{} optimization. Given that we use the Stable Diffusion~\cite{Rombach:2022StableDiffusion}, we compute the source latent at viewpoint $v$ by the encoder $\mathcal{E}$ expressed as $\B{x}^{\text{src}}_{0,v} = \mathcal{E}(I_v)$. Similarly, the target latent is also computed by encoding a current rendering output $\B{x}_{0,v}^{\text{tgt}} = \mathcal{E}(g(\theta; c_v))$, where $g(\theta; c_v)$ is the NeRF rendering output at viewpoint $v$. To edit NeRF, we randomly select $v$ and update the NeRF parameter $\theta$ through the \Ours{} optimization using the finetuned diffusion model $\hat{\Veps}_\phi$. 

\paragraph{Refinement Stage.}
While \Ours{} generally produces satisfactory results by updating a given NeRF scene to align with a given target prompt, it can occasionally introduce undesired artifacts into the output. Inspired by DreamBooth3D~\cite{raj2023dreambooth3d}, we take further steps to refine the \Ours{} output using a reconstruction loss with image-to-image translation output images. Specifically, we use SDEdit~\cite{Meng:2022SDEdit} for the image-to-image translation. We denote a SDEdit operator by $\mathcal{S}(I, t; \Veps_\phi)$, where $I$ is an input image, $t$ is a denoising starting timestep and $\Veps_\phi$ is a learned noise predictor. To begin the refinement stage, we first render an updated NeRF scene from the \Ours{} optimization stage at the viewpoints $\{v\}$ used in the previous stage, resulting in an image dataset $\{\tilde{I}^0_v\}$. Similar to Instruct-NeRF2NeRF~\cite{Haque:2023InstructNeRF}, we iteratively update the image dataset using SDEdit: 
$\tilde{I}^i_v = \mathcal{S}(\tilde{I}^0_v, t; \hat{\Veps}_\phi)$, where $\tilde{I}^i_v$ is the $i$-th updated reference image at viewpoint $v$, the result of SDEdit using the finetuned noise predictor $\hat{\Veps}_\phi$. Note that we use the initial image dataset $\{\tilde{I}_v^0\}$ when making updates. This approach ensures that the updated images do not stray too far from their original images.

Using the iteratively updated image dataset, we update $\theta$ by a reconstruction loss:
\begin{align}
    \mathcal{L}_{\text{recon}} = \Vert g(\theta; c_v) - \tilde{I}^i_v \Vert_2^2.
\end{align}

\begin{figure*}
\dummyfig{1\textwidth}{0.4\textwidth}{An overview of our pipeline.}
\caption{An overview of our pipeline.}
\end{figure*}

